Temporal Representation Alignment: Successor Features Enable Emergent Compositionality in Robot Instruction Following

Effective task representations should facilitate compositionality, such that after learning a variety of basic tasks, an agent can perform compound tasks consisting of multiple steps simply by composing the representations of the constituent steps together. While this is conceptually simple and appealing, it is not clear how to automatically learn representations that enable this sort of compositionality. We show that learning to associate the representations of current and future states with a temporal alignment loss can improve compositional generalization, even in the absence of any explicit subtask planning or reinforcement learning. We evaluate our approach across diverse robotic manipulation tasks as well as in simulation, showing substantial improvements for tasks specified with either language or goal images.

==> data.tex <==
\makeatletter

\newarray\tasks\readarray{tasks}{\langbox{put the corn and sushi on plate}&\langbox{sushi and mushroom in bowl}&\langbox{corn, banana, and sushi in bowl}&\langbox{put the spoons on towels}&\langbox{put the spoons on the plates}&\langbox{open the drawer}&\langbox{mushroom in drawer}&\langbox{close drawer}&\langbox{fold cloth into the center}&\langbox{sweep to the right}&\langbox{take the item out of the drawer}&\langbox{corn on plate then sushi in pot}&\langbox{move bell pepper and sweep towel}}

\def\getlang#1{\tasks(#1)\gdef\i{#1}}



\pgfplotstableread{build/msedata.dat}\mse@data

\def\nodata{\rule[0.5ex]{1em}{1pt}}

\def\processmod#1{
    \pgfplotstablecreatecol[create col/assign/.code={\pgfkeys{/pgf/number format/.cd,fixed,precision=2,fixed zerofill=true}
        \getthisrow{#1_average}\tmp
        \edef\tmp{\tmp}
        \edef\nan{NaN}
        \ifx\tmp\nan
            \def\entry{\nodata}
        \else
            \getthisrow{#1_average}\avg
            \getthisrow{#1_stderr}\std
            \pgfmathprintnumberto\avg{\avg}\pgfmathprintnumberto\std{\std}
            \edef\entry{$\avg\,\pm\,\std$}
        \fi
        \pgfkeyslet{/pgfplots/table/create col/next content}\entry
    }]{#1}{\mse@data}
}
\processmod{language}
\processmod{image}

\pgfplotstabletranspose[colnames from={method},columns={image,language},input colnames to=modality]\mse@data\mse@data



\typeout{No file "build/total.dat".}
\pgfplotstableread{eval.dat}\eval@data
\pgfplotstableread{build/total.dat}\total@data

\newcount\nextbar
\def\methodbar#1#2{
    \providecommand\style{}
    \advance\nextbar by 1
    \newcount\i
    \expandafter\gdef\csname li@\the\nextbar\endcsname{}
    \pgfplotstablegetrowsof{\total@data}
    \edef\n{\pgfplotsretval}
    { \loop
        \edef\coordindex{\the\i}
        \expanded{\noexpand\pgfplotstablegetelem{\coordindex}{method}}\of\total@data
        \def\target{#1}
        \ifx\pgfplotsretval\target
            \expanded{\noexpand\pgfplotstablegetelem{\coordindex}{mean}}\of\total@data
            \let\avg\pgfplotsretval
            \expanded{\noexpand\pgfplotstablegetelem{\coordindex}{stderr}}\of\total@data
            \expandafter\gdef\csname li@\the\nextbar\endcsname{\nameuse{l@#1}}
            \expanded{\noexpand
                \addplot[fill=#2,\style,pattern color=#2] coordinates {(\avg,\the\nextbar) +- (\pgfplotsretval,0.0)};
            }
        \else
            \advance\i by 1
            \ifnum\i<\n
        \fi
        \repeat
    }
}

\pgfplotsset{
    keep/.style={
        y filter/.code={\ifnum\coordindex=#1\else\def\pgfmathresult{}\fi}
    },
}

\pgfplotstableread{msedata.dat}\orig@msedata

\pgfplotstableread{build/total.dat}\total@data

\def\pmformat#1#2{\fontsize{7}{7}\selectfont$\text{#1}^{\fontsize{4}{4}\selectfont(\pm\text{#2})}$}

\def\missing{0/0}\def\get#1{\edef\a{{\the\numexpr \i-1}}\expandafter\pgfplotstablegetelem\a{#1}\of\eval@data\ifx\pgfplotsretval\missing{\setbox0=\hbox{\stats0/0\relax}\makebox[\wd0][c]{\nodata}}\else\expandafter\stats\pgfplotsretval\relax\fi}\def\stats#1/#2\relax{\pgfmathparse{#1/#2}\pgfmathprintnumberto[fixed,precision=2,zerofill,assume math mode=true]{\pgfmathresult}\avg\pgfmathparse{sqrt(\pgfmathresult*(1-\pgfmathresult)/#2}\pgfmathprintnumberto[fixed,precision=1,zerofill,assume math mode=true]{\pgfmathresult}{\std}\pmformat\avg\std}

\begin{figure}[htb!]
    \usefont{T1}{ppl}{m}{n}
    \centering\begin{subfigure}{.9\linewidth}
        \resizebox{\linewidth}{!}{\begin{tikzpicture}\pgfplotsset{every axis/.append style={width=\linewidth,xmin=0,xmax=.95,height=4.5cm,enlarge y limits={abs=0.5cm},}}\namedef{l@LCBC}{LCBC}\namedef{l@GRIF-L}{GRIF}\namedef{l@OURS-L}{\textbf{\Method (Ours)}}\namedef{l@OCTO-L}{Octo}\namedef{l@AWR+GRIF-L}{AWR}\begin{axis}[ytick=data,xbar,bar width=0.4cm,error bars/x dir=both,error bars/x explicit,error bars/error bar style={line width=1pt,black},error bars/error mark options={line width=1pt,black,rotate=90},x axis line style={-},y axis line style={draw=none},yticklabels from table={\total@data}{method},xlabel={Success Rate},every axis plot/.append style={draw=none,bar shift=0pt},title={Instruction Following Performance},name=overall eval,ytick={0,...,6},yticklabel={\pgfmathparse{\tick}\pgfmathtruncatemacro\trunc{\pgfmathresult}\nameuse{li@\trunc}}]\methodbar{OURS-L}{theme1}\methodbar{AWR+GRIF-L}{theme2}\methodbar{GRIF-L}{theme7}\methodbar{OCTO-L}{theme5}\methodbar{LCBC}{theme0}\end{axis}\end{tikzpicture}}\caption{Language instruction tasks}\end{subfigure}\par
    \medskip
    \begin{subfigure}{.9\linewidth}\begin{adjustbox}{width=\linewidth}
            \begin{tikzpicture}\pgfplotsset{every axis/.append style={width=\linewidth,xmin=0,xmax=.95,height=4.5cm,enlarge y limits={abs=0.5cm},}}\namedef{l@GCBC}{GCBC}\namedef{l@GRIF-I}{GRIF}\namedef{l@OURS-I}{\textbf{\Method (Ours)}}\namedef{l@OCTO-I}{Octo}\namedef{l@AWR+GRIF-I}{AWR}\begin{axis}[ytick=data,xbar,bar width=0.4cm,error bars/x dir=both,error bars/x explicit,error bars/error bar style={line width=1pt,black},error bars/error mark options={line width=1pt,black,rotate=90},x axis line style={-},y axis line style={draw=none},yticklabels from table={\total@data}{method},xlabel={Success Rate},every axis plot/.append style={draw=none,bar shift=0pt},title={Goal Reaching Performance},name=overall eval,ytick={0,...,6},yticklabel={\pgfmathparse{\tick}\pgfmathtruncatemacro\trunc{\pgfmathresult}\nameuse{li@\trunc}}]\methodbar{OURS-I}{theme1}\methodbar{AWR+GRIF-I}{theme2}\methodbar{GRIF-I}{theme7}\methodbar{OCTO-I}{theme5}\methodbar{GCBC}{theme0}\end{axis}\end{tikzpicture}
        \end{adjustbox}\caption{Goal-image conditioned tasks}\end{subfigure}\caption{Aggregated performance on compositional generalization tasks, consisting of instruction-following and goal-reaching tasks.}\end{figure}

\makeatother


